Entanglement is Necessary for Optimal Quantum Property Testing

There has been a surge of progress in recent years in developing algorithms for testing and learning quantum states that achieve optimal copy complexity. Unfortunately, they require the use of entangled measurements across many copies of the underlying state and thus remain outside the realm of what is currently experimentally feasible. A natural question is whether one can match the copy complexity of such algorithms using only independent---but possibly adaptively chosen---measurements on individual copies. We answer this in the negative for arguably the most basic quantum testing problem: deciding whether a given $d$-dimensional quantum state is equal to or $\epsilon$-far in trace distance from the maximally mixed state. While it is known how to achieve optimal $O(d/\epsilon^2)$ copy complexity using entangled measurements, we show that with independent measurements, $\Omega(d^{4/3}/\epsilon^2)$ is necessary, even if the measurements are chosen adaptively. This resolves a question of Wright. To obtain this lower bound, we develop several new techniques, including a chain-rule style proof of Paninski's lower bound for classical uniformity testing, which may be of independent interest.

==> moments.tex <==
%!TEX root = ./new_quantum_paninski.tex

\section{Haar Tail Bounds}
\label{subsec:tails}

In this section we prove two key estimates, Theorems~\ref{thm:moments} and~\ref{thm:rho_tail}, which will be crucial to our final proof of Theorem~\ref{thm:main}.

\begin{theorem}
	For any POVM $\calM$, let $p$ denote the distribution over outcomes from measuring $\mm$ with $\calM$, and let $\gamma > 0$ be an absolute constant. Define the random variable \begin{equation}
		K^{\U,\U'}_{\calM} \triangleq \E[x\sim p]*{\left(g^{\U}_{\calM}(x) + g^{\U'}_{\calM}(x)\right)^2}
	\end{equation} Then for any $n = o(d^2/\epsilon^2)$, we have that \begin{equation}
		\E[{\U,\U'}]*{\left(1 + \gamma\cdot K^{\U,\U'}_{\calM}\right)^n} \le \exp(O(\gamma n \epsilon^2/d))
		\label{eq:Kdef}
	\end{equation}
	\label{thm:moments}
\end{theorem}

\begin{example}
	When $\calM$ is an orthogonal POVM by an orthonormal basis of $\C^d$, then $p$ is uniform over $[d]$ and $K^{\U,\U'}_{\calM}$ is simply $\frac{\epsilon^2}{d}\sum^d_{i=1}(\delta(\U_i) + \delta(\U'_i))^2$. It follows from Fact~\ref{fact:randomunitvector} that this has expectation $\epsilon^2/d$. By Lemma~\ref{lem:basicZtail}, this quantity concentrates well enough that by integration by parts, \eqref{eq:Kdef} would hold in this case.
\end{example}

\begin{proof}[Proof of Theorem~\ref{thm:moments}]

Let $\calM$ be an arbitrary POVM. We first show a bound on $\E[\U,\U']{K^{\U,\U'}_{\calM}}$. The following lemma can be interpreted as a generalization of Fact~\ref{fact:randomunitvector} which is used in the analysis of our mixedness tester in Section~\ref{subsec:tester}.

\begin{lemma}
	$\E[\U,\U']{K^{\U,\U'}_{\calM}} \le \frac{\epsilon^2}{d+1}$.
	\label{lem:secondmoment}
\end{lemma}

\begin{proof}
	Note that $K^{\U,\U'}_{\calM} = 2\E[x\sim p]*{g^{\U}_{\calM}(x)^2} + 2\rho^{\U,\U'}_{\calM}$. We will suppress the subscripts for the rest of this proof. Clearly we have that $\E[\U,\U']{\rho^{\U,\U'}} = 0$, so it remains to bound $\E[x\sim p,\U,\U']*{g^{\U}(x)^2}$. Let $\tau^*\in\Sym_2$ denote the non-identity permutation. For any fixed $x$, by Lemma~\ref{lem:weincalc}, \begin{align}
		\E[\U]{g^{\U}(x)^2} &= \sum_{\sigma,\tau\in\Sym_2}\iprod{\X}_{\tau}\iprod{\hatM_x}_{\sigma}\Wg(\sigma\tau^{-1},d) \\
		&= \iprod{\X}_{\tau^*} \left(\Tr(\hatM_x^2)\cdot \Wg(e,d) + \Tr(\hatM_x)^2\cdot \Wg(\tau^*,d)\right) \\
		&= \epsilon^2\cdot d\cdot\left(\frac{1}{d^2 - 1}\Tr(\hatM_x^2) - \frac{1}{d(d^2-1)}\right) \le \frac{\epsilon^2}{d+1},\label{eq:gzsingle}
	\end{align} where the second step follows by the fact that $\iprod{\X}_{\tau} = \epsilon^2\cdot d\cdot \bone{\tau= \tau^*}$, and the last step follows by the fact that $\Tr(\hatM_x^2) \le 1$. As \eqref{eq:gzsingle} holds for any outcome $x$, $\E[x\sim p,\U,\U']{g^{\U}(x)^2} \le \frac{\epsilon^2}{d+1}$ as desired.
\end{proof}

We next show the following tail bound, which can be interpreted as a generalization of Lemma~\ref{lem:basicZtail} which is also used in the analysis of our mixedness tester in Section~\ref{subsec:tester}:

\begin{lemma}
	There are absolute constants $c,c'>0$ such that for any $t > c \epsilon^2/d$, 
	\begin{equation}
		\Pr[\U,\U'\sim\calD]*{K^{\U,\U'}_{\calM} > c\epsilon^2/d + t} \le \exp(-c' t d^2/\epsilon^2))
	\end{equation}	
	\label{lem:Ztail}
\end{lemma}

\begin{proof}
	We wish to apply Theorem~\ref{thm:deusexmachina}. We will show that $F: (\U,\U')\mapsto \left(K^{\U,\U'}_{\calM}\right)^{1/2}$ is $L$-Lipschitz for $L = O(\epsilon/\sqrt{d})$. As $\E{F(\U,\U')} \le \E[\U,\U']*{K^{\U,\U'}_{\calM}}^{1/2} \le \frac{\epsilon}{\sqrt{d+1}}$ by Jensen's and Lemma~\ref{lem:secondmoment}, this would imply that for any $s > 0$, \begin{equation}
		\Pr[\U\sim\calD]*{F(\U,\U') > \frac{\epsilon}{\sqrt{d+1}} + s} \le e^{-d^2s^2/12\epsilon^2},
	\end{equation} from which the lemma would follow by taking $s = \sqrt{t}$.

	To show Lipschitz-ness, note that \begin{equation}
		F(\U,\U') = \E[x\sim p]*{\left(g^{\U}_{\calM}(x) + g^{\U'}_{\calM}(x)\right)^2} \le \E[x\sim p]*{g^{\U}_{\calM}(x)^2}^{1/2} + \E[x\sim p]*{g^{\U'}_{\calM}(x)^2}^{1/2},
	\end{equation} so the proof is complete given Lemma~\ref{lem:Glipschitz} below.
\end{proof}

\begin{lemma}
	The function $G: \U\mapsto \E[x\sim p]*{g^{\U}_{\calM}(x)^2}^{1/2}$ is $O(\epsilon/\sqrt{d})$-Lipschitz.
	\label{lem:Glipschitz}
\end{lemma} 

\begin{proof}
	Take any $\U,\V\in U(d)$ and note that by triangle inequality, \begin{equation}
		G(U) - G(V) \le \E[x\sim p]*{\left(g^{\U}_{\calM}(x) - g^{\V}_{\calM}(x)\right)^2}^{1/2},
	\end{equation} so it suffices to show \begin{equation}
		\E[x\sim p]*{\left(g^{\U}_{\calM}(x) - g^{\V}_{\calM}(x)\right)^2} \le O(\epsilon^2/d)\cdot\norm{\U - \U'}^2_{HS}.
		\label{eq:wantlipschitz}
	\end{equation}
	$\A\triangleq \U^{\dagger}\X\U - \V^{\dagger}\X\V$ is Hermitian, so write its eigendecomposition $\A = \W^{\dagger}\Sig\W$. Then \begin{equation}
		g^{\U}_{\calM}(x) - g^{\V}_{\calM}(x) = \iprod*{\hatM_x, \A} = \iprod*{\W \hatM_x \W^{\dagger},\Sig} = \iprod*{\diag(\W\hatM_x\W^{\dagger}),\Sig},
	\end{equation} so we may assume without loss of generality that $\A$ and $\hatM_x$ are diagonal, in which case by Jensen's, \begin{equation}
		\left(g^{\U}_{\calM}(x) - g^{\V}_{\calM}(x)\right)^2 = \iprod{\hatM_x,\A}^2 = \left(\sum^d_{i=1} (\hatM_x)_{ii}\A_{ii}\right)^2 \le \sum^d_{i=1} (\hatM_x)_{ii}\A^2_{ii}.
	\end{equation}
	Recalling that $p(x) = \Tr(M_x)/d$, the left-hand side of \eqref{eq:wantlipschitz} becomes \begin{align}
		\frac{1}{d}\int \Tr(M_x)\cdot \iprod{\hatM_x,\A}^2 \d\mu &= \frac{1}{d}\int \sum_{i\in[d]} \Tr(M_x)\cdot (\hatM_x)_{ii}\A^2_{ii}\d \mu \\
		&= \frac{1}{d}\norm{\A}^2_{HS} = \frac{1}{d}\norm{\U^{\dagger}\X(\U - \V) + (\V - \U)^{\dagger}\X\V}^2_{HS} \le \frac{2\epsilon^2}{d}\norm{\U - \V}^2_{HS},
	\end{align} completing the proof of \eqref{eq:wantlipschitz}.
\end{proof}

To complete the proof of Theorem~\ref{thm:moments}, we would like to apply Fact~\ref{fact:stieltjes} to the random variable $Z\triangleq 1 + \gamma\cdot K^{\U,\U'}_{\calM}$ and the function $f(Z)\triangleq Z^n$. Note that this random variable is nonnegative and upper bounded by $1+C\cdot\gamma\cdot \epsilon^2$ for some absolute constant $C > 0$. So \begin{align}
	\E[\U,\U']*{\left(1 + \gamma K^{\U,\U'}_{\calM}\right)^n} &\le 2(1 + O(\gamma\epsilon^2/d))^n + \int^{1 + C\gamma\epsilon^2}_{1 + c\gamma\epsilon^2/d}nt^{n-1}\cdot e^{-\Omega(t\cdot d^2/\epsilon^2)}\ \d t \\
	&\le 2(1 + O(\gamma\epsilon^2/d))^n + \int^{\infty}_0 nt^{n-1}\cdot e^{-\Omega(t\cdot d^2/\epsilon^2)}\ \d t \\
	&= 2(1 + O(\gamma\epsilon^2/d))^n + n!\cdot O(\epsilon^2/d^2)^n \\
	&\le e^{O(\gamma\epsilon^2 n/d)},
\end{align} where in the last step we used that $n!\cdot O(\epsilon^2/d^2)^n$ is negligible when $n = o(d^2/\epsilon^2)$
\end{proof}

As discussed earlier, the next estimate is the ``quantum analogue'' of tail bounds for binomials.

\rhotail*

\begin{proof}
	Define $G$ as in Lemma~\ref{lem:Glipschitz}. Fix any $\U'$ and consider the function $F_{\U'}: \U\mapsto \rho^{\U,\U'}_{\calM}$. 
	First note that \begin{equation}
		\E[\U]{F_{\U'}(\U)} = \E[x\sim p]{g^{\U'}_{\calM}(x)\cdot \E[\U]{g^{\U}_{\calM}(x)}}= 0
	\end{equation} by Part~\ref{fact:zero} of Fact~\ref{fact:basic}.
	Next, note that by Cauchy-Schwarz, \begin{equation}
		F_{\U'}(\U) - F_{\U'}(\V) \le \E[x\sim p]*{\left(g^{\U}_{\calM}(x) - g^{\V}_{\calM}(x)\right)^2}^{1/2} \cdot G(\U'),
	\end{equation}
	which by \eqref{eq:wantlipschitz} is $O(\epsilon/\sqrt{d})\cdot G(\U')$-Lipschitz.
	So for any fixed $\U'$, Theorem~\ref{thm:deusexmachina} implies \begin{equation}
		\Pr[\U]{\abs{F_{\U'}(\U)} > t} \le \exp\left(-C\cdot \frac{d^2t^2}{\epsilon^2 G(\U')^2}\right)\label{eq:integrand}
	\end{equation} for some absolute constant $C> 0$. We would like to integrate over $\U'$ to get a tail bound for $\rho^{\U,\U'}_{\calM}$ as a function of both $\U$ and $\U'$.

	To this end, we can apply Fact~\ref{fact:stieltjes} to the random variable $Y\triangleq G(\U') \in [0,\epsilon]$. Recall from \eqref{eq:gzsingle} and Jensen's that $\E{Y}\le\epsilon/\sqrt{d+1}$. Furthermore, by Lemma~\ref{lem:Glipschitz} and Theorem~\ref{thm:deusexmachina}, there is an absolute constant $C'>0$ such that \begin{equation}
		\Pr{Y > \epsilon/\sqrt{d+1} + s} \le \exp\left(-C'd^2s^2/\epsilon^2\right).\label{eq:Yconc}
	\end{equation}
	So we can take the parameters in Fact~\ref{fact:stieltjes} as follows: set $a \triangleq 2\epsilon/\sqrt{d+1}$, tail bound function $\tau(x)\triangleq \exp\left(-C'\cdot \frac{d^2}{\epsilon^2}\left(x - \frac{\epsilon}{\sqrt{d+1}}\right)^2\right)$ for absolute constant $C'>0$, and $f(Y)\triangleq \exp\left(-C\cdot\frac{d^2t^2}{\epsilon^2 Y^2}\right)$. By \eqref{eq:integrand}, $\Pr[\U,\U']*{\abs*{\rho^{\U,\U'}_{\calM}}>t} \le \E{f(Y)}$, and by Fact~\ref{fact:stieltjes}, \begin{equation}
		\E{f(Y)} \le 2\exp\left(-\Omega(d^3t^2/\epsilon^4)\right) + \int^{\epsilon}_{2\epsilon/\sqrt{d+1}} \frac{2C d^2t^2}{\epsilon^2 x^3} \exp\left(-\frac{d^2}{\epsilon^2} \left(\frac{Ct^2}{x^2} + C'\left(x - \frac{\epsilon}{\sqrt{d+1}}\right)^2\right)\right) \ \d x.
	\end{equation} Note that by AM-GM, for $x\ge 2\epsilon/\sqrt{d+1}$ we have that \begin{equation}
		\frac{Ct^2}{x^2} + C'\left(x - \frac{\epsilon}{\sqrt{d+1}}\right)^2 \ge 2t\cdot (C\cdot C')^{1/2}\cdot \left(1 - \frac{\epsilon/\sqrt{d+1}}{x}\right) \ge t\cdot (C\cdot C')^{1/2}.
	\end{equation} We conclude that \begin{equation}
		\Pr[\U,\U']*{\abs*{\rho^{\U,\U'}_{\calM}}>t} \le 2\exp\left(-\Omega(d^3t^2/\epsilon^4)\right) + \frac{2Cd^{7/2}t^2}{\epsilon^4}\cdot \exp\left(-\Omega\left(d^2t/\epsilon^2\right)\right).
	\end{equation} In particular, for $t \ge \Omega(\epsilon^2/d^{1.99})$, we have that \begin{equation}
		\Pr[\U,\U']*{\abs*{\rho^{\U,\U'}_{\calM}}>t} \ge \exp\left(-\Omega\left(\Min{\frac{d^3t^2}{\epsilon^4}}{\frac{d^2t}{\epsilon^2}}\right)\right)
	\end{equation} as claimed.
\end{proof}
